Controllability Analysis of Multi-Modal Acoustic Particle Manipulation in One-Dimensional Standing Waves

Acoustic manipulation in microfluidic devices enables contactless handling of biological cells for Lab-on-Chip applications. This paper analyzes the controllability of multi-particle systems in a one-dimensional acoustic standing wave system using multi-modal actuation. By modeling the system as a nonlinear control system, we analyze its global and local controllability, quantifying these properties in terms of mode numbers. Our results show that sufficient modes enable dense reachability sets, while mode mixing with 10 modes grants a strict notion of controllability to 80\% of the state space in a two-particle system. These findings offer theoretical insights for designing acoustic manipulation algorithms, supporting efficient control in biomedical applications.

==> backup.tex <==
We relied on Euler's method to approximate the system dynamics described in (\ref{sys:n_1d}) and simulate the state-transition from any state $x$ under any mode mixture $w$ for a fixed timestep $\Delta_t$. Note that this approach requires us to discretize the problem in time.

\begin{equation} \label{simulation_euler}
    x^{(w)}[t+1] = x[t] + \dot{x}^{(w)}[t]\Delta_t
\end{equation}

Since we are using the mode-mixing assumption (\ref{sys:relax:n_1d}) we have that the set of all possible next states will be a convex set, $C(x)$.
\begin{equation}
   C(x) = \{ x + \dot{x} \Delta_t, \forall \dot{x} \in  \cco (F(x)) \}
\end{equation}

Let us now define the concept of a \textit{reachable state}: $x$ is said to be reachable if $x \in \interior C(x)$, that is, if there exists a neighborhood of $x$ that can be completely reached from $x$ in the next timestep. Note that the reachability of a state is closely linked to the number of modes we make available in the process, since it directly affects $F(x)$. One example is shown in Figure \ref{fig:example_cvxhull}, where a given state $x$ is not reachable with three modes, but becomes so with the addition of the fourth one. Our simulation is able to find $C(x)$ for any given state $x$ and, with a simple operation, we can check if $x \in \interior C(x)$ and, thus, to determine its reachability.

\begin{figure}[h]
    \centering
    \includegraphics[width=0.49\linewidth]{pic/example_mode3.png}
    \includegraphics[width=0.49\linewidth]{pic/example_mode4.png}
    \caption{}
    \label{fig:example_cvxhull}
\end{figure}

Using this definition of reachability, we can infer that we have full controllability in regions consisting solely of reachable states. In order to determine where these regions may lie, we overlaid a fine grid of states on top of the entire space and determined the reachability of each of its members. Note that this is a crude approximation of the system's controllability, given that (1) we are using Euler's method to estimate its dynamics, (2) two non-reachable states can still reach each other by moving through a longer path, and (3) the grid must be sufficiently fine if we want to assert that neighboring reachable states can actually reach each other and compose a reachable region. In our experiment, we used two particles with radius X,Y, and a grid spacing of Z. The results can be seen in Figure 7.
